Towards Handling Unconstrained User Preferences in Dialogue

A user input to a schema-driven dialogue information navigation system, such as venue search, is typically constrained by the underlying database which restricts the user to specify a predefined set of preferences, or slots, corresponding to the database fields. We envision a more natural information navigation dialogue interface where a user has flexibility to specify unconstrained preferences that may not match a predefined schema. We propose to use information retrieval from unstructured knowledge to identify entities relevant to a user request. We update the Cambridge restaurants database with unstructured knowledge snippets (reviews and information from the web) for each of the restaurants and annotate a set of query-snippet pairs with a relevance label. We use the annotated dataset to train and evaluate snippet relevance classifiers, as a proxy to evaluating recommendation accuracy. We show that with a pretrained transformer model as an encoder, an unsupervised/supervised classifier achieves a weighted F1 of .661/.856.

==> reviews.tex <==


Reviewer 1:
1. It isn't mentioned in the paper whether one or multiple annotators did this, and what the agreement here is like.
>>> We already have this information in the paper in Section 3.3 last line.

2. It would also be interesting to see how the ResQS with negative reviews would have performed.
>>> I think we are not expected to this now. Also, as our current assumption we do not expect to find relevant information for the queries in negative reviews.

3. The concepts were largely well explained, with minor typographical errors (e.g. dialogues systems, servers) and grammar inconsistencies not really getting in the way of understanding.
>>> Changed dialogues systems to dialogue systems in section 2
>>> Changed servers to serves section 4.1

4. However, it was slightly confusing to me that "two unsupervised and one transfer learning methods" in section 3.3 was not elaborated upon, and immediately followed by a diagram (Fig. 2) for four different methods which were discussed in section 4.
>>> Have added footnote 4 in page 6 to make this clear.

5. It took me a while to figure out how the 210 additional query-snippet pairs for the queries which specified database fields were arrived at. I believe they were chosen "using three methods to select five methods per query", i.e. 14 * 3 * 5 = 210, but even now I'm not entirely sure.
>>> Addded an additional sentence in section 3.3 " Thus by using three methods to select five snippets per query for additional 14 queries we extend... "


Reviewer 2:
1. The weakness of the paper is not the authors work, it is that the description of the work is confusing and lacking a simple definition of how they use terminology to the point where it becomes unclear what the authors mean when they talk about snippet relevance, about query-snippet annotation and what was meant by subjective and objective property.

2. I had difficulties to understand the experiment description.

3. The paper would probably improve if it would receive another review pass towards missing articles and a consistent usage of English past tense and presence.
>>> I have tried my best but I am very bad at using articles.

4. I also would recommend a very simple explanation of how the user queries, the collected snippets, the relevance annotations, and in which the system would eventually retrieve the answers from refer to each other.


5. Section 3.3 to 4 are essential to understand the approaches the authors describe but are not clear.

6. towards what entity are the subjective and objective property attributes subjective and objectives?



Reviewer 3:

1.  the whole approach is reminiscent of (conversational) QA, in that external text sources are employed to provide answers to a user query, in this case based on an extractive process. It would perhaps be useful to make this connection with QA approaches more explicit, and point to what distinguishes (if anything) those approaches and the model presented in the paper.

>>> Our target currently is  to find a matching restaurant for which we assume similarity between query and snippets is enough. Unlike QA we do not need to extract (or sometimes even generate) specific text from passages that match the query. Thus, we might have to focus on improving the similarity aspects rather than the answer retrieval aspects of QA.

>>>I have not made any correction to the paper regarding this and I'm not sure if this is required.



2.  the paper mentions that the long-term goal is to develop a hybrid system that would be able to seamlessly handle both queries that are "slot-based" as well as "out-of-slot". How would the system decide whether to trigger the traditional dialogue state tracking + dialogue policy or the IE-based model? That's a tricky question, and it would be useful to write a few words about it.

>>> I'm currently unsure about this and would require more reading.


3.  Since the model is used to determine the relevance of a given snippet, why not use IE-based metrics such as MRR, cumulative gain or similar (as detailed in https://amitness.com/2020/08/information-retrieval-evaluation/) in the evaluation section? It seems like evaluating the model in terms of F1 on binary relevance is a quite crude way of evaluating the model performance.

>>> Although we do not present MRR results but we present similar metrics in form of percentage relevant and avg number of relevant snippets in Table 2.

----------------------------------------------------------------------------------------------


SUBMISSION: 13
TITLE: Towards Handling Unconstrained User Preferences in Dialogue


----------------------- REVIEW 1 ---------------------
SUBMISSION: 13
TITLE: Towards Handling Unconstrained User Preferences in Dialogue
AUTHORS: Suraj Pandey, Svetlana Stoyanchev and Rama Doddipatla

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
This work presents part of an approach to expand the knowledge base of a conversational agent.

A small structured dataset is augmented with unstructured data, and snippet relevance models that can rank the elements of the dataset for a fixed number of queries are trained so that recommendations can be made; that is, a recommender system is built based on an augmented dataset.

Future work promises to integrate this recommender into an actual dialogue system for user testing, so this is where the work is relevant to the theme of the conference.

I found the approach to rank snippets interesting, as the model outputs were ultimately manually annotated as relevant/not-relevant (section 5.1), which adds a layer of subjectivity to the ranking. It isn't mentioned in the paper whether one or multiple annotators did this, and what the agreement here is like. This may have led to different conclusions on whether Cos-TF-IDF or Cos-Bert produced the higher percentage of relevant snippets.

On the whole, the reasoning seems all right, but the strength of the evidence could be improved somewhat.

It would also be interesting to see how the ResQS with negative reviews would have performed.
----------- Clarity of writing / Quality of presentation -----------
SCORE: 4 (good)
----- TEXT:
The concepts were largely well explained, with minor typographical errors (e.g. dialogues systems, servers) and grammar inconsistencies not really getting in the way of understanding.

However, it was slightly confusing to me that "two unsupervised and one transfer learning methods" in section 3.3 was not elaborated upon, and immediately followed by a diagram (Fig. 2) for four different methods which were discussed in section 4.

It took me a while to figure out how the 210 additional query-snippet pairs for the queries which specified database fields were arrived at. I believe they were chosen "using three methods to select five methods per query", i.e. 14 * 3 * 5 = 210, but even now I'm not entirely sure.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 13
TITLE: Towards Handling Unconstrained User Preferences in Dialogue
AUTHORS: Suraj Pandey, Svetlana Stoyanchev and Rama Doddipatla

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
What are the main strengths and weaknesses?
The paper describes research around a relevant task - extending dialog systems towards a more natural human-like conversation flow. The introduction, related work section, the final discussion and the references are good and comprehensive and provide a good motivation and justification for the authors work.

The weakness of the paper is not the authors work, it is that the description of the work is confusing and lacking a simple definition of how they use terminology to the point where it becomes unclear what the authors mean when they talk about snippet relevance, about query-snippet annotation and what was meant by subjective and objective property.

Is the content novel?
The content is another approach towards making human-machine dialogs more natural. This is a relevant and modern topic.

Is the experimental validation sound?
I had difficulties to understand the experiment description.

Are references adequate?
yes

Is the paper relevant to the scope of IWSDS?
yes
----------- Clarity of writing / Quality of presentation -----------
SCORE: 2 (poor)
----- TEXT:
The paper would probably improve if it would receive another review pass towards missing articles and a consistent usage of English past tense and presence.

I also would recommend a very simple explanation of how the user queries, the collected snippets, the relevance annotations, and in which the system would eventually retrieve the answers from refer to each other.
Section 3.3 to 4 are essential to understand the approaches the authors describe but are not clear.

towards what entity are the subjective and objective property attributes subjective and objectives?



----------------------- REVIEW 3 ---------------------
SUBMISSION: 13
TITLE: Towards Handling Unconstrained User Preferences in Dialogue
AUTHORS: Suraj Pandey, Svetlana Stoyanchev and Rama Doddipatla

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The paper presents an approach to handle "out-of-slot" user preferences in information navigation dialogues, using a IR mechanism that takes advantage of text snippets collected on the web. The paper comes along with an annotated dataset and a empirical evaluation of various models for relevance classification (both unsupervised and supervised variants).

The paper is interesting and addresses an important problem, namely how to deal with user queries that fall outside of the predefined slots that have been defined for the task.

I only have a couple of comments:
- the whole approach is reminiscent of (conversational) QA, in that external text sources are employed to provide answers to a user query, in this case based on an extractive process. It would perhaps be useful to make this connection with QA approaches more explicit, and point to what distinguishes (if anything) those approaches and the model presented in the paper.
- the paper mentions that the long-term goal is to develop a hybrid system that would be able to seamlessly handle both queries that are "slot-based" as well as "out-of-slot". How would the system decide whether to trigger the traditional dialogue state tracking + dialogue policy or the IE-based model? That's a tricky question, and it would be useful to write a few words about it.
- Since the model is used to determine the relevance of a given snippet, why not use IE-based metrics such as MRR, cumulative gain or similar (as detailed in https://amitness.com/2020/08/information-retrieval-evaluation/) in the evaluation section? It seems like evaluating the model in terms of F1 on binary relevance is a quite crude way of evaluating the model performance.
----------- Clarity of writing / Quality of presentation -----------
SCORE: 4 (good)

